Quantum Relational Hoare Logic

We present a logic for reasoning about pairs of interactive quantum programs - quantum relational Hoare logic (qRHL). This logic follows the spirit of probabilistic relational Hoare logic (Barthe et al. 2009) and allows us to formulate how the outputs of two quantum programs relate given the relationship of their inputs. Probabilistic RHL was used extensively for computer-verified security proofs of classical cryptographic protocols. Since pRHL is not suitable for analyzing quantum cryptography, we present qRHL as a replacement, suitable for the security analysis of post-quantum cryptography and quantum protocols. The design of qRHL poses some challenges unique to the quantum setting, e.g., the definition of equality on quantum registers. Finally, we implemented a tool for verifying proofs in qRHL and developed several example security proofs in it.

==> macros.tex <==
\makeatletter

\newcommand\pagelabel[1]{\phantomsection\label{#1}}

\DeclareRobustCommand\sagelink[1]{%
  \let\SAGECELLLINK\undefined
  \InputIfFileExists{#1.sagelink}{}{}%
  \typeout{XXX:\meaning\SAGECELLLINK}%
  \ifx\SAGECELLLINK\undefined\expandafter\@firstoftwo
  \else\expandafter\@secondoftwo\fi
  {\TODOQ{Create #1.sagelink}}%
  {\edef\@tempa{\noexpand\href{\SAGECELLLINK}}%
    \@tempa}}

\mdfdefinestyle{proofstyle}{%
  backgroundcolor=black!4!white,
  innertopmargin=3pt,
  innerbottommargin=3pt,
  innerleftmargin=3pt,
  innerrightmargin=3pt,
  linewidth=0pt
}

\mdfdefinestyle{claimproofstyle}{%
  backgroundcolor=black!8!white,
  innertopmargin=0pt,
  innerbottommargin=3pt,
  innerleftmargin=3pt,
  innerrightmargin=3pt,
  leftmargin=10pt,
  rightmargin=10pt,
  % linewidth=0pt
}

\newenvironment{proof}[1][]{%
  \begin{mdframed}[style=proofstyle]%
    \begin{trivlist}%
    \item \textit{Proof\ifx\proof#1\proof\else\ #1\fi. }%
    }{
      \qed\global\let\qed\qedmacro
    \end{trivlist}
  \end{mdframed}}%

\newenvironment{claimproof}{%
  \let\qedbox\qedboxclaim
  \begin{mdframed}[style=claimproofstyle]%
    \begin{trivlist}%
    \item \textit{Proof of claim. }%
    }{
      \qed\global\let\qed\qedmacro
    \end{trivlist}
  \end{mdframed}}%

\newenvironment{claimproofstart}{%
  \let\qedbox\qedboxclaim
  \begin{mdframed}[style=claimproofstyle]%
    \begin{trivlist}%
    \item \textit{Proof of claim. }%
    }{
    \end{trivlist}
  \end{mdframed}}%

\newenvironment{claimproofend}{%
  \let\qedbox\qedboxclaim
  \begin{mdframed}[style=claimproofstyle]%
    \begin{trivlist}%
    \item%
    }{
      \qed\global\let\qed\qedmacro
    \end{trivlist}
  \end{mdframed}}%



% \showafter{year}{month}{day}{text} evaluates to {text} starting from year/month/day
\newcommand\showafter[4]{%
  \ifnum\year>#1\relax
    #4% today.year > args.year
  \else
    \ifnum\year=#1\relax
    % today.year = args.year
      \ifnum\month>#2\relax
      % today.month > args.month
        #4%
      \else
        \ifnum\month=#2\relax
        % today.month = args.month
          \ifnum\day>#3\relax
          % today.day >= args.day
            #4%
          \else
            \ch@removeduplicatespace
          \fi
        \else
          \ch@removeduplicatespace
        \fi
      \fi
    \else
      \ch@removeduplicatespace
    \fi
  \fi}


\let\textttOLD\texttt
\def\texttt#1{\textttOLD{\frenchspacing #1}}

\makeatletter
\newcommand\qedboxclaim{\ensuremath\diamond}
\newcommand\qedbox{\m@th$\Box$}
\newcommand\qedmacro{\hfill\qedbox}
\global\let\qed\qedmacro
\newcommand\skipqed{\global\let\qed\empty}
\newcommand\mathQED{\tag*{\qedbox}\skipqed}
\newcommand\txtrel[1]{\stackrel{\hskip-1in\text{\tiny#1}\hskip-1in}}
\newcommand\eqrefrel[1]{\txtrel{\eqref{#1}}}
\newcommand\starrel{\txtrel{$(*)$}}
\newcommand\tristarrel{\txtrel{$\scriptscriptstyle (\!*\!*\!*\!)$}}
\newcommand\fourstarrel{\txtrel{$\scriptscriptstyle (\!*\!*\!*\!*\!)$}}
\newcommand\starstarrel{\txtrel{$(**)$}}
\newcommand\boardpic[1]{\par{\centering\includegraphics[keepaspectratio=true,width=\hsize,height=2.5in]{#1}\par}}
\newcommand\rimplies{\DOTSB\;\Longleftarrow\;}
\newcommand\sublemmaref[2]{\autoref{#1}\,\eqref{sub#1:#2}}
\DeclareRobustCommand\autorefshort[1]{%
  \def\lemmaautorefname{Lem.\!}%
  \autoref{#1},
  p.\,\pageref{#1}}
\newcommand\bit{\{0,1\}}
\newcommand\bits[1]{\bit^{#1}}

\def\parenthesis@resizecommand@open{}
\def\parenthesis@resizecommand@close{}
\def\parenthesis@#1#2#3#4#5{%
  \global\let\parenthesis@resizecommand@open\empty
  \global\let\parenthesis@resizecommand@close\empty
  #1#3%
  {#5}%
  #2#4%
}
\DeclareRobustCommand\parenthesis[3]{%
  \expandafter\expandafter\expandafter
  \parenthesis@\expandafter\expandafter\expandafter{\expandafter\parenthesis@resizecommand@open\expandafter}\expandafter{\parenthesis@resizecommand@close}{#1}{#2}{#3}}


% #1=bigl #2=bigr #3=( #4=txt #5=) #6=txt #7=( #8=txt #9=)
\def\double@parenthesis@#1#2#3#4#5#6#7#8#9{%
  \global\let\parenthesis@resizecommand@open\empty
  \global\let\parenthesis@resizecommand@close\empty
  #1#3{#4}#2#5%
  {#6}%
  #1#7{#8}#2#9%
}

\DeclareRobustCommand\doubleParenthesis[7]{%
  \expandafter\expandafter\expandafter
  \double@parenthesis@\expandafter\expandafter\expandafter{\expandafter\parenthesis@resizecommand@open\expandafter}\expandafter{\parenthesis@resizecommand@close}{#1}{#2}{#3}{#4}{#5}{#6}{#7}}


\DeclareRobustCommand\resize@next@paren[2]{%
  \gdef\parenthesis@resizecommand@open{#1}%
  \gdef\parenthesis@resizecommand@close{#2}%
}

\newcommand\paren{\parenthesis()}
\newcommand\braces{\parenthesis\{\}}

\newcommand\pb{\resize@next@paren\bigl\bigr}
\newcommand\pbb{\resize@next@paren\biggl\biggr}
\newcommand\plr{\resize@next@paren\left\right}
\newcommand\pB{\resize@next@paren\Bigl\Bigr}

\newlistof{rule}{rule}{{List of rules}}
\renewcommand\cftruletitlefont{\section*}
\newcommand\rulestrut{}
\newcommand\rulespace{}
\newcommand\RULE[4][]{%
  \inferrule[\rulestrut{#2\ifx\norulelemmalink\undefined
    \textsuperscript{\normalfont\tiny[\autorefshort{rule-lemma:#2}]}\fi}%
    \refstepcounter{rule}%
    \label{rule:#2}%
    \index{#2@\textsc{#2} (rule)}%
    \addcontentsline{rule}{rule}{\textsc{#2}%
      \ifx\@nil#1\@nil\else\space -- #1\fi}
  ]{#3}{#4}\rulespace%  
}
\newcommand\RULEX[4][]{%
  \inferrule[\rulestrut{#2}%
      \ifx\@nil#1\@nil\else\space -- #1\fi]{#3}{#4}\rulespace%  
}
\newenvironment{ruleblock}{%
  \begin{center}%
    \def\rulestrut{\vrule height 1.3\baselineskip width 0pt\relax}%
    \def\rulespace{\qquad}%
    \noindent
  }{%
  \end{center}}
  
\newcommand\refrule[1]{\hyperref[rule:#1]{\hbox{\textsc{#1}}} rule}
\newcommand\ruleref[1]{\hyperref[rule:#1]{rule \hbox{\textsc{#1}}}}
\newcommand\rulerefx[1]{\hyperref[rule:#1]{\hbox{\textsc{#1}}}}
\newcommand\Ruleref[1]{\hyperref[rule:#1]{Rule \hbox{\textsc{#1}}}}


%\newcommand\butter[2]{\basis{#1}\bra{#2}}
%\newcommand\selfbutter[2]{\proj{\basis{#1}{#2}}}

%\declare{macro=\varcard, code=\kappa, 
%  description={Upper bound for cardinality of variable types}}

\declare{macro=\abs, argspec=[1], code=\parenthesis\lvert\rvert{#1},
  placeholder=\abs x, nopage=true,
  description=Absolute value of $x$ / cardinality of set $x$}
%\declare{macro=\babs, argspec=[1], code={\bigl\lvert#1\bigr\rvert}, 
%  variantof=\abs}

\declare{macro=\qu, argspec=[1], code=#1^\mathsf{qu},
  placeholder=\qu V,
  description={Quantum variables in $V$}}
\declare{macro=\cl, argspec=[1], code=#1^\mathsf{cl},
  placeholder=\cl V,
  description={Classical variables in $V$}}

\declare{macro=\fv, code=\mathit{fv},
  placeholder=\fv(e),
  description={Free variables in an expression $e$ (or program)}}

\declare{macro=\typev, argspec=[1], code=\mathsf{Type}_{#1},
  placeholder=\typev v,
  description={Type of variable $v$}}
\declare{macro=\types, argspec=[1], code=\mathsf{Type}^\mathsf{set}_{#1},
  placeholder=\types X,
  description={Type of a set $V$ of variables}}
\declare{macro=\typel, argspec=[1], code=\mathsf{Type}^\mathsf{list}_{#1},
  placeholder=\typel V,
  description={Type of a list $V$ of variables}}
\declare{macro=\typee, argspec=[1], code=\mathsf{Type}^\mathsf{exp}_{#1},
  placeholder=\typee e,
  description={Type of an expression $e$}}

\declare{macro=\denotee, argspec=[2], code=\parenthesis\llbracket\rrbracket{#1}_{#2},
  placeholder=\denotee em,
  description={Denotation of a classical expression $e$, evaluated on classical memory $m$}}

%\declare{macro=\denoteex, argspec=[1], code=\llbracket#1\rrbracket,
%  variantof=\denotee}

\declare{macro=\bc, code=\mathbf c, nopage=true,
  variable=true,
  description={A program}}
\declare{macro=\bd, code=\mathbf d, nopage=true,
  variable=true,
  description={A program}}
\newcommand\be{\mathbf e}

\declare{macro=\denotc, argspec=[1], code={\parenthesis\llbracket\rrbracket{#1}},
  placeholder={\denotc \bc},
  description={Denotation of a program $\bc$}}
\declare{macro=\denotcl, argspec=[1], code={\parenthesis\llbracket\rrbracket{#1}_\mathbf{class}},
  placeholder={\denotcl \bc},
  description={Classical denotation of a program $\bc$}}

\declare{macro=\Skip, code=\mathbf{skip},
  description={Program that does nothing}}

\declare{macro=\langif, argspec=[3], code={\mathbf{if}\ #1\ \mathbf{then}\ #2\ \mathbf{else}\ #3},
  placeholder=\langif e{c_1}{c_2},
  description=Statement: If (conditional)}
%\declare{macro=\langifx, argspec=[2], code={\mathbf{if}\ #1\ \mathbf{then}\ #2},
%  variantof=\langif}
%\declare{macro=\langifkw, code={\mathbf{if}},
%  variantof=\langif}

\declare{macro=\while, argspec=[2], code={\mathbf{while}\ #1\ \mathbf{do}\ #2},
  placeholder=\while ec,
  description=Statement: While loop}
%\declare{macro=\whilekw, code={\mathbf{while}},
%  variantof=\while}
\newcommand\whilep[2]{\while{#1}{\{#2\}}}

\declare{macro=\sample, argspec=[2], code={#1\stackrel{{\scriptstyle{}\$}}\leftarrow #2},
  placeholder=\sample \xx e,
  description={Statement: Sample $\xx$ according to distribution $e$}}

\declare{macro=\Qinit, argspec=[2],
  code={#1\stackrel{{\scriptstyle{\text{\bfseries\sffamily q}}}}\leftarrow #2},
  % code={\mathbf{init}\ #1\leftarrow #2},
  % code={#1\twoheadleftarrow#2},
  placeholder=\Qinit{\qq_1\dots \qq_n}{e},
  description={Statement: Initialize $\qq_1,\dots,\qq_n$ with quantum state $e$}}
\declare{macro=\Qapply, argspec=[2], code={\mathbf{apply}\ #1\ \mathbf{to}\ #2},
  placeholder=\Qapply{\qq_1\dots \qq_n}{U},
  description={Statement: Apply unitary/isometry $U$ to quantum registers $\qq_1\dots \qq_n$}}

\declare{macro=\Qmeasure, argspec=[3], code={#1 \leftarrow \mathbf{measure}\ #2\ \mathbf{with}\ #3},
  placeholder=\Qmeasure{\xx}{\qq_1\dots\qq_n}{e},
  description={Statement: Measure quantum variables $\qq_1\dots\qq_n$ with measurement $e$}}

\declare{macro=\bool, code=\mathbb B,
  description={Booleans. $\bool=\{\true,\false\}$}}

\declare{macro=\elltwo, argspec=[1], code={\ell^2(#1)},
  placeholder=\elltwo B,
  description={Hilbert space with basis indexed by $B$}}
\declare{macro=\elltwov, argspec=[1], code={\ell^2\parenthesis[]{#1}},
  placeholder=\elltwov V,
  description={$\elltwo{\types V}$ -- Hilbert space with basis $\types V$}}

\declare{macro=\ellone, argspec=[1], code={\mathbf D(#1)},
  placeholder=\ellone B,
  description={Distributions on $B$}}
\declare{macro=\ellonev, argspec=[1], code={\mathbf D[#1]},
  placeholder=\ellonev V,
  description={$\ellone{\types V}$ -- Distributions on $\types V$}}

\declare{macro=\iso, argspec=[1], code=\mathbf{Iso}(#1),
  placeholder={\iso{X,Y}, \iso X},
  description={Isometries from $\elltwo X$ to $\elltwo Y$ (on $\elltwo X$)}}
\declare{macro=\isov, argspec=[1], code={\mathbf{Iso}[#1]},
  placeholder={\isov{V,W}, \iso V},
  description={Isometries from $\elltwov V$ to $\elltwov W$ (on $\elltwov V$)}}

\declare{macro=\uni, argspec=[1], code=\mathbf{U}(#1),
  placeholder={\uni{X,Y}, \uni X},
  description={Unitaries from $\elltwo X$ to $\elltwo Y$ (on $\elltwo X$)}}
\declare{macro=\univ, argspec=[1], code={\mathbf{U}[#1]},
  placeholder={\univ{V,W}, \uni V},
  description={Unitaries from $\elltwov V$ to $\elltwov W$ (on $\elltwov V$)}}

\declare{macro=\distr, argspec=[1], code=\mathbf D^{\leq1}(#1),
  placeholder=\distr X,
  description={Sub-probability distributions over $X$}}
\declare{macro=\distrv, argspec=[1], code=\mathbf D^{\leq1}[#1],
  placeholder=\distrv V,
  description={Sub-probability distributions over variables $V$}}

\declare{macro=\setC, code=\mathbb C,
  description={Complex numbers}}
\declare{macro=\setR, code=\mathbb R,
  description={Real numbers}}
\declare{macro=\setRpos, code=\mathbb R_{\geq0},
  description={Non-negative real numbers}}

\declare{macro=\tracecl, argspec=[1], code=\mathbf T(#1),
  placeholder={\tracecl X},
  description=Trace class operators on $\elltwo X$}
\declare{macro=\tracepos, argspec=[1], code=\mathbf T^+(#1),
  placeholder={\tracepos X},
  description=Positive trace class operators on $\elltwo X$}
\declare{macro=\tensor, code=\otimes,
  placeholder={A\otimes B},
  description={Tensor product of vectors/operators $A$ and $B$}}

\declare{macro=\traceclv, argspec=[1], code=\mathbf T[#1],
  placeholder={\traceclv V},
  description=Trace class operators on $\elltwov V$}
\declare{macro=\traceposv, argspec=[1], code=\mathbf T^+[#1],
  placeholder={\traceposv V},
  description=Positive trace class operators on $\elltwov V$}
\declare{macro=\traceclcq, argspec=[1], code=\mathbf T_{\mathit{cq}}[#1],
  placeholder={\traceclcq V},
  description=Trace class cq-operators on $\elltwov V$}

\declare{macro=\pointdistr, argspec=[1],
  code={\delta_{#1}},
  placeholder=\pointdistr{x},
  description={Point distribution: returns $x$ with probability $1$}}

\declare{macro=\restricte, argspec=[1], code=\mathord\downarrow_{#1},
  placeholder=\restricte e(\rho),
  description={Restrict state/distribution $\rho$ to the case $e=\true$ holds}}
\newcommand\restrictno[2]{#1}

\declare{macro=\seq, argspec=[2], code=#1;#2,
  placeholder=\bc;\bd,
  description={Sequential composition of programs}}


% \declare{macro=\pointstate, argspec=[2],
%   code={\delta_{#1}(#2)},
%   placeholder=\delta_V(x),
%   description={Point distribution as density operator}}
\newcommand\pointstate[2]{\proj{\basis{#1}{#2}}}

\declare{macro=\true, code=\mathtt{true}, nopage=true,
  description={Truth value ``true''}}
\declare{macro=\false, code=\mathtt{false}, nopage=true,
  description={Truth value ``false''}}

\declare{macro=\traceposcq, argspec=[1], code=\mathbf T^+_{\mathit{cq}}[#1],
  placeholder={\traceposcq V},
  description=Positive trace class cq-operators on $\elltwov V$}

\declare{macro=\qlift, argspec=[1], code=\mathsf{lift}\paren{#1},
  placeholder=\qlift\mu,
  description=Transforms a distribution $\mu$ into a density operator}

\declare{macro=\lift, argspec=[2], code={#1\textrm\guillemotright#2},
  placeholder=\lift AQ,
  description={Lifts operator or subspace to variables $Q$}}

%\declare{macro=\compl, argspec=[1], code=#1^{\complement},
%  placeholder=\compl X,
%  description=Complement of the set $X$}

\declare{macro=\calE, code=\mathcal E, variable=true,
  description=A superoperator}

\declare{macro=\bounded, argspec=[1], code=\mathbf B(#1),
  placeholder={\bounded{X,Y}},
  description=Bounded linear operators from $\elltwo X$ to $\elltwo Y$}
\declare{macro=\boundedleq, argspec=[1], code=\mathbf B^{\leq1}(#1),
  placeholder={\boundedleq{X,Y}},
  description=Bounded linear operators with operator norm $\leq1$}
\declare{macro=\boundedv, argspec=[1], code=\mathbf B[#1],
  placeholder=\boundedv{V,W},
  description={Bounded linear operators from $\elltwov V$ to $\elltwo W$}}

\declare{macro=\idv, argspec=[1], code=\mathit{id}_{#1},
  placeholder=\idv V,
  description=Identity on $\elltwov V$ or on $\boundedv V$}
\declare{macro=\id, code=\mathit{id},
  description=Identity}

\declare{macro=\adj, argspec=[1], code=#1^*,
  placeholder={\adj A},
  description={Adjoint of the operator $A$}}

%\newcommand\basisOLD[1]{\lvert #1\rangle}
\declare{macro=\basis, argspec=[2], code={\parenthesis\lvert\rangle{#2}_{\!\scriptscriptstyle{#1}}},
  placeholder={\basis{} b, \basis V b},
  description={Basis vector in Hilbert space $\elltwov V$}}
%\declare{macro=\bra, argspec=[1], code={\langle #1\lvert},
%  placeholder=\bra b,
%  description={$\adj{\basis b}$, adjoint of basis vector $\basis b$}}

% \declare{macro=\hoarev, argspec=[4], code={\{#1\}#2\{#3\}^{#4}},
%   placeholder=\hoarev F\bc GV,
%   description={Possibilistic Hoare judgement (variables $V$ omitted if clear)}}
% \declare{macro=\hoare, argspec=[3], code={\{#1\}#2\{#3\}},
%   variantof=\hoarev}

\declare{macro=\rhl, argspec=[4],
  % code={\{#1\}#2\pmb\sim#3\{#4\}},
  code={\doubleParenthesis\{{#1}\}{#2\pmb\sim#3}\{{#4}\}},
  placeholder=\rhl F\bc{\bc'} G,
  description={Quantum relational Hoare judgment}}
\declare{macro=\rhlfirst, argspec=[4],
  % code={\{#1\}#2\pmb\sim#3\{#4\}},
  code={\doubleParenthesis\{{#1}\}{#2\pmb\sim#3}\{{#4}\}_\mathsf{nonsep}},
  placeholder=\rhlfirst F\bc{\bc'} G,
  description={qRHL judgment, non-separable definition}}
\declare{macro=\rhlunif, argspec=[4],
  % code={\{#1\}#2\pmb\sim#3\{#4\}},
  code={\doubleParenthesis\{{#1}\}{#2\pmb\sim#3}\{{#4}\}_\mathsf{uniform}},
  placeholder=\rhlunif F\bc{\bc'} G,
  description={qRHL judgment, uniform definition}}
%\declare{macro=\rhlv, argspec=[6], code={\{#1\}#2\sim#3\{#4\}^{#5,#6}},
%  variantof=\rhlv}
\declare{macro=\prhl, argspec=[4],
  % code={\{#1\}#2\pmb\sim#3\{#4\}},
  code={\doubleParenthesis\{{#1}\}{#2\pmb\sim#3}\{{#4}\}_\mathsf{class}},
  placeholder=\prhl F\bc{\bc'} G,
  description={pRHL judgement (classical)}}

\declare{macro=\partr, argspec=[2], 
  code=\mathord{\operatorname{tr}^{\scriptscriptstyle[#1]}_{\scriptscriptstyle #2}},
  placeholder=\partr VW(\rho),
  description={Partial trace, keeping variables $V$, dropping variables $W$}}

\declare{macro=\im, code=\operatorname{im},
  placeholder=\im A,
  description={Image of $A$}}
\declare{macro=\dom, code=\operatorname{dom},
  placeholder=\dom f,
  description={Domain of $f$}}

\declare{macro=\norm, argspec=[1], code={\parenthesis\lVert\rVert{#1}},
  placeholder=\norm x, description={$\ell_2$-norm of vector $x$, or operator-norm}}
%\declare{macro=\bnorm, argspec=[1], code={\bigl\lVert#1\bigr\rVert}, variantof=\norm}

\declare{macro=\tr, code=\operatorname{tr},
  placeholder=\tr M,
  description={Trace of matrix/operator $M$}}

\declare{macro=\CL, argspec=[1], code=\mathfrak{Cla}\parenthesis[]{#1},
  placeholder=\CL e,
  description={Classical predicate meaning $e=\true$}}

\declare{macro=\SPAN, code={\operatorname{span}},
  placeholder=\SPAN A,
  description={Span, smallest subspace containing $A$}}
\newcommand\SPANO[1]{\SPAN\{#1\}}

\declare{macro=\quanteq, code={\equiv_\mathsf{quant}},
  placeholder=X_1\quanteq X_2,
  description={Equality of quantum variables $X_1$ and $X_2$}}

\declare{macro=\proj, argspec=[1], code={\mathsf{proj}\parenthesis(){#1}},
  placeholder=\proj x,
  description={Projector onto $x$, i.e., $x\adj x$}}

\declare{macro=\prafter, argspec=[3], code={\Pr\parenthesis[]{#1 : #2(#3)}},
  placeholder=\prafter e\bc\rho,
  description={Probability that $e$ holds after running $\bc$ on initial state $\rho$}}

\declare{macro=\Urename, argspec=[1], code={U_{\mathit{rename},#1}},
  placeholder=\Urename{\sigma},
  description={Unitary: Renames variables according to bijection $\sigma$}}


\declare{macro=\Erename, argspec=[1], code={\calE_{\mathit{rename},#1}},
  placeholder=\Erename{\sigma},
  description={cq-superoperator: Renames variables according to bijection $\sigma$}}

\declare{macro=\subst, argspec=[2], code=#1#2,
  placeholder={\subst e\sigma, \subst\bc\sigma},
  description={Apply variable renaming $\sigma$ to expression $e$}}

\declare{macro=\substi, argspec=[2], code=#1\{#2\},
  placeholder=\substi e{f/\xx},
  description={Substitute $f$ for variable $\xx$ in $e$}}

\declare{macro=\restrict, argspec=[2], code=#1|_{#2},
  placeholder=\restrict fM,
  description={Restriction of function $f$ to domain $M$}}

\declare{macro=\xx, code=\mathbf x,
  description={A classical program variable}}
\declare{macro=\yy, code=\mathbf y,
  description={A classical program variable}}
%\declare{macro=\zz, code=\mathbf z,
%  description={A classical program variable}}
\declare{macro=\qq, code=\mathbf q,
  description={A quantum program variable}}
\newcommand\rr{\mathbf r}
% \declare{macro=\rr, code=\mathbf r,
%   description={A quantum program variable}}


\declare{macro=\upd, argspec=[3], code={#1(#2:=#3)},
  placeholder=\upd fxy,
  description={Function update, i.e., $(\upd fxy)(x)=y$}}


\declare{macro=\assign, argspec=[2], code={#1\leftarrow #2},
  placeholder=\assign xe,
  description={Program: assigns expression $e$ to $x$}}

\declare{macro=\suppd, code=\operatorname{supp},
  placeholder=\suppd \mu,
  description={Support of distribution $\mu$}}
\declare{macro=\suppo, code=\operatorname{\mathbf{supp}},
  placeholder=\suppo M,
  description={Support of an operator $M$}}

\declare{macro=\marginal, argspec=[2], code={\mathsf{marginal}_{#1}\parenthesis(){#2}},
  placeholder=\marginal i\mu,
  description={$i$-th marginal distribution of $\mu$ (for $\mu\in\distr{X\times Y}$, $i=1,2$)}}

\declare{macro=\orth, argspec=[1], code={#1^\bot},
  placeholder=\orth S,
  description={Orthogonal complement of subspace $S$}}

% \declare{macro=\calH, code=\mathcal H,
%   description={A Hilbert space}}

% \declare{macro=\pinv, argspec=[1], code=#1^+,
%   placeholder=\pinv A,
%   description={Moore-Penrose pseudoinverse}}

\declare{macro=\idx, argspec=[1], code=\operatorname{idx}_{#1},
  placeholder={\idx 1\bc, \idx 1 e},
  description={Add index $1$ to every variables in $\bc$ or $e$}}

\declare{macro=\Meas, argspec=[2], code={\mathbf{Meas}(#1,#2)},
  placeholder=\Meas DE,
  description={Projective measurements on $\elltwo E$ with outcomes in $D$}}

\declare{macro=\Uvarnames, argspec=[1], code=U_{\mathit{vars},#1},
  placeholder=\Uvarnames{Q},
  description={Canonical isomorphism between $\elltwo{\typel Q}$
    and $\elltwov{\types Q}$ for a list $Q$}}

% \declare{macro=\leftim, argspec=[1], code=\overleftarrow\im\, #1,
%   placeholder=\leftim R,
%   description={Left image of relation $R$}}

% \declare{macro=\rightim, argspec=[1], code=\overrightarrow\im\, #1,
%   placeholder=\rightim R,
%   description={Right image of relation $R$}}

\declare{macro=\spaceat, argspec=[2], code=#1\div#2,
  placeholder=\spaceat A\psi,
  description={Part of $A$ containing $\psi$}}

\declare{macro=\memuni, argspec=[1], code=#1,
  placeholder=\memuni{m_1m_2},
  description={Union (concatenation) of memories $m_1$, $m_2$}}

\declare{macro=\powerset, argspec=[1], code=2^{#1},
  placeholder=\powerset M,
  description={Powerset of $M$}}

\declare{macro=\floor, argspec=[1], code=\parenthesis\lfloor\rfloor{#1},
  placeholder=\floor x,
  description={$x$ rounded down to the next integer}}

%\declare{macro=\sampleset, code=\in_{\scriptstyle{}\$},
%  placeholder=x\sampleset M,
%  description={$x$ uniformly sampled from $M$}}
\declare{macro=\AdvROR, code=\mathrm{Adv}_\mathrm{ROR},
  placeholder=\AdvROR^{A_1A_2}(\eta),
  description={Advantage of adversary $A_1,A_2$ in ROR-OT-CPA game with security parameter $\eta$}}
\declare{macro=\AdvPRG, code=\mathrm{Adv}_\mathrm{PRG},
  placeholder=\AdvPRG^{A}(\eta),
  description={Advantage of adversary $A$ in PRG-OT-CPA game with security parameter $\eta$}}
\declare{macro=\Time, code=\mathrm{Time},
  placeholder=\Time(A),
  description={Worst-case runtime of $A$}}


\declare{macro=\circexp, code=\circ_e,
  placeholder=a \circexp b,
  description={Composition of expressions $a,b$ as relations}}
\declare{macro=\circrel, code=\circ,
  placeholder=R_1 \circrel R_2,
  description={Composition of relations}}

\declare{macro=\setN, code=\mathbb N,
  description={Natural numbers}}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "qrhl"
%%% TeX-PDF-mode: t 
%%% End: 

%  LocalWords:  Powerset

